CROW: Code Diversification for WebAssembly

The adoption of WebAssembly has rapidly increased in the last few years as it provides a fast and safe model for program execution. However, WebAssembly is not exempt from vulnerabilities that could be exploited by side channels attacks. This class of vulnerabilities that can be addressed by code diversification. In this paper, we present the first fully automated workflow for the diversification of WebAssembly binaries. We present CROW, an open-source tool implementing this workflow. We evaluate CROW's capabilities on 303 C programs and study its use on a real-life security-sensitive program: libsodium, a cryptographic library. Overall, CROWis able to generate diverse variants for 239 out of 303,(79%) small programs. Furthermore, our experiments show that our approach and tool is able to successfully diversify off-the-shelf cryptographic software (libsodium).

==> parts/algorithm.tex <==

\vspace{0.5cm}
\begin{algorithm}[H]

\SetKwData{optimizations}{optimizations}
\SetKwData{variants}{variants}
\SetKwData{newvar}{newvar}
\SetKwData{subset}{subset}
\SetKwFunction{so}{sop}
\SetKwFunction{apply}{apply}
\SetKwFunction{to}{to}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

\Input{program $P$, superoptimizer \so}
\Output{Set of program variants \variants }
$\optimizations \leftarrow \so(P)$ \;
$\variants \leftarrow \emptyset$ \;
\ForEach{ $\subset \in \mathcal{P}(\optimizations)$ } {
    \newvar $\leftarrow$ \apply \subset \to $P$\;
    $\variants \leftarrow \variants \cup \newvar$\;
}

\caption{Generating program variants by leveraging the superoptimizer search strategy}
\label{alg:generation}
\end{algorithm}

==> tables/rq1.tex <==
\newcolumntype{M}{>{\begin{varwidth}{2.5cm}}l<{\end{varwidth}}}

\begin{table*}
\begin{scriptsize}
    \begin{tabular}{  l r r r r }
    \hline
    Name & \# Blocks & \# Variants & \# Unique & \% Unique  \\
    \hline
 p1 & 3 & 1821 & 281 & 15.43 \% \\ 
 \rowcolor{rowcolor!20} p2 & 23 & 12100 & 270 & 2.23 \% \\ 
 p3 & 29 & 2504 & 254 & 10.14 \% \\ 
 p4 & 59 & 1746 & 223 & 12.77 \% \\ 
 p5 & 15 & 18001 & 187 & 1.04 \% \\ 
 p6 & 15 & 9901 & 179 & 1.81 \% \\ 
 p7 & 59 & 1561 & 142 & 9.10 \% \\ 
 p8 & 10 & 4001 & 132 & 3.30 \% \\ 
 p9 & 24 & 10461 & 121 & 1.16 \% \\
 p10 & 23 & 1702 & 89 & 5.23 \% \\ 
 p11 & 35 & 1851 & 87 & 4.70 \% \\ 
 p12 & 30 & 1465 & 83 & 5.67 \% \\ 
 p13 & 3 & 1825 & 77 & 4.22 \% \\ 
 p14 & 3 & 1821 & 76 & 4.17 \% \\ 
 p15 & 13 & 1728 & 74 & 4.28 \% \\ 
 p16 & 82 & 241 & 72 & 29.88 \% \\ 
 p17 & 22 & 1623 & 65 & 4.00 \% \\ 
 p18 & 17 & 16580 & 64 & 0.39 \% \\ 
 p19 & 44 & 1386 & 60 & 4.33 \% \\ 
 p20 & 15 & 401 & 51 & 12.72 \% \\ 
 p21 & 68 & 501 & 51 & 10.18 \% \\ 
 p22 & 3 & 241 & 46 & 19.09 \% \\ 
 p23 & 65 & 1021 & 45 & 4.41 \% \\ 
 p24 & 4 & 2081 & 44 & 2.11 \% \\ 
 p25 & 23 & 2042 & 43 & 2.11 \% \\ 
 p26 & 16 & 1633 & 43 & 2.63 \% \\ 
 p27 & 8 & 241 & 37 & 15.35 \% \\ 
 p28 & 6 & 924 & 33 & 3.57 \% \\ 
 p29 & 55 & 989 & 32 & 3.24 \% \\ 
 p30 & 11 & 102 & 32 & 31.37 \% \\ 
 p31 & 25 & 361 & 31 & 8.59 \% \\ 
 p32 & 7 & 241 & 26 & 10.79 \% \\ 
 p33 & 23 & 1401 & 26 & 1.86 \% \\ 
 p34 & 5 & 1219 & 25 & 2.05 \% \\ 
 p35 & 34 & 281 & 24 & 8.54 \% \\ 
 p36 & 21 & 601 & 24 & 3.99 \% \\ 
 p37 & 54 & 141 & 23 & 16.31 \% \\ 
 p38 & 14 & 5633 & 23 & 0.41 \% \\ 
 p39 & 33 & 2961 & 23 & 0.78 \% \\ 
 p40 & 23 & 181 & 23 & 12.71 \% \\ 
 p41 & 4 & 221 & 23 & 10.41 \% \\ 
 p42 & 4 & 7641 & 23 & 0.30 \% \\ 
 p43 & 20 & 61 & 22 & 36.07 \% \\ 
 p44 & 9 & 281 & 22 & 7.83 \% \\ 
 p45 & 47 & 2481 & 22 & 0.89 \% \\ 
 p46 & 17 & 1005 & 22 & 2.19 \% \\ 
 p47 & 29 & 811 & 22 & 2.71 \% \\ 
 p48 & 37 & 221 & 21 & 9.50 \% \\ 
 p49 & 43 & 804 & 21 & 2.61 \% \\ 
 p50 & 6 & 61 & 21 & 34.43 \% \\ 
 p51 & 44 & 321 & 21 & 6.54 \% \\ 
 p52 & 19 & 161 & 21 & 13.04 \% \\ 
 p53 & 29 & 341 & 21 & 6.16 \% \\ 
 p54 & 11 & 18521 & 20 & 0.11 \% \\ 
 p55 & 51 & 61 & 17 & 27.87 \% \\ 
 p56 & 6 & 61 & 16 & 26.23 \% \\ 
 p57 & 14 & 361 & 16 & 4.43 \% \\ 
 p58 & 28 & 61 & 15 & 24.59 \% \\ 
 p59 & 17 & 41 & 15 & 36.59 \% \\ 
 p60 & 20 & 141 & 14 & 9.93 \% \\ 
 p61 & 12 & 181 & 13 & 7.18 \% \\ 
 p62 & 24 & 41 & 13 & 31.71 \% \\ 
 p63 & 50 & 441 & 12 & 2.72 \% \\ 
 p64 & 19 & 42 & 10 & 23.81 \% \\ 
 p65 & 50 & 61 & 8 & 13.11 \% \\ 
 p66 & 17 & 21 & 6 & 28.57 \% \\ 
 p67 & 20 & 21 & 5 & 23.81 \% \\ 
 p68 & 29 & 21 & 4 & 19.05 \% \\ 
 \rowcolor{rowcolor!20} p69 & 7 & 22 & 4 & 18.18 \% \\ 
 p70 & 40 & 21 & 4 & 19.05 \% \\ 
 \rowcolor{rowcolor!20} p71 & 74 & 21 & 3 & 14.29 \% \\ 
 p72 & 15 & 21 & 3 & 14.29 \% \\ 
 p73 & 6 & 21 & 3 & 14.29 \% \\ 
 p74 & 37 & 21 & 3 & 14.29 \% \\ 
 p75 & 5 & 2 & 2 & 100.00 \% \\ 
 p76 & 24 & 21 & 2 & 9.52 \% \\ 
 p77 & 19 & 11 & 2 & 18.18 \% \\ 
 p78 & 5 & 21 & 2 & 9.52 \% \\ 
 p79 & 4 & 21 & 2 & 9.52 \% \\ 
 p80 & 3 & 21 & 2 & 9.52 \% \\ 
 p81 & 17 & 81 & 2 & 2.47 \% \\ 
 \rowcolor{rowcolor!20} p82 & 79 & 61 & 2 & 3.28 \% \\ 
 
 
    \end{tabular}
\end{scriptsize}
    \caption{Programs with more than one unique variant. The columns are structured as follows, program name, number of identified pure code blocks, number of variants, number of unique variants and the percentage of unique variants.}
    \label{tables:rq1}
\end{table*}

==> tables/stage1_table.tex <==
\begin{table}[t]

\resizebox{0.5\textwidth}{!}{
  \begin{tabular}{l r r} 
  
      \hline
      Program name & Program variants & Different program variants  \\
      %    &              &     &                   &          &           \\
      \hline\hline
      Multiplication tables      & 26069        & 3224 \\
        \hline 
      Law of cosines - triples      & 82283        & 2103 \\
        \hline 
      URL decoding      & 32        & 16 \\
        \hline 
      Roots of unity      & 129        & 16 \\
        \hline 
      Mian-Chowla sequence      & 44688        & 16 \\
        \hline 
      Holidays related to Easter      & 17        & 9 \\
        \hline 
      100 doors      & 33        & 8 \\
        \hline 
      N'th      & 65        & 8 \\
        \hline 
      Hilbert curve      & 9        & 8 \\
        \hline 
      Tokenize a string with escaping      & 11        & 7 \\
        \hline 
      Middle three digits      & 5        & 4 \\
        \hline 
      Show Ascii table      & 33        & 4 \\
        \hline 
      Combinations      & 5        & 4 \\
        \hline 
      Evaluate binomial coefficients      & 5        & 4 \\
        \hline 
      Sailors, coconuts and a monkey problem      & 5        & 4 \\
        \hline 
      Permutations-Rank of a permutation      & 9        & 4 \\
        \hline 
      Babbage problem      & 45        & 4 \\
        \hline 
      Fibonacci sequence      & 9        & 4 \\
        \hline 
      Burrows–Wheeler transform      & 37544        & 4 \\
        \hline 
      Cartesian product of two or more lists      & 54632        & 4 \\
        \hline 
      Sierpinski triangle      & 192        & 3 \\
        \hline 
      Magic squares of singly even order      & 9        & 3 \\
        \hline 
      99 Bottles of Beer      & 5        & 3 \\
        \hline 
      Largest number divisible by its digits      & 4        & 2 \\
        \hline 
      Thiele's interpolation formula      & 3        & 2 \\
        \hline 
      Knuth shuffle      & 3        & 2 \\
        \hline 
      Best shuffle      & 3        & 2 \\
        \hline 
      Chebyshev coefficients      & 65        & 2 \\
        \hline 
      Hofstadter-Conway 10,000 sequence      & 17        & 2 \\
        \hline 
      Vampire number      & 3        & 2 \\
        \hline 
      Remove duplicate elements      & 5        & 2 \\
        \hline 
      Zeckendorf number representation      & 3        & 2 \\
        \hline 
      Day of the week      & 5        & 2 \\
        \hline 
      Gray code      & 3        & 2 \\
        \hline 
      Sort numbers lexicographically      & 3        & 2 \\
        \hline 
      Compare a list of strings      & 9        & 2 \\
        \hline 
      Sorting algorithms-Sleep sort      & 5        & 2 \\
        \hline 
      Total circles area      & 68        & 2 \\
        \hline 
      Ramsey's theorem      & 33        & 2 \\
        \hline 
      Quickselect algorithm      & 4097        & 2 \\
        \hline 
      Sorting algorithms-Bubble sort      & 129        & 2 \\
        \hline 
      Longest increasing subsequence      & 33        & 2 \\
        \hline 
      Fast Fourier transform      & 3        & 2 \\
        \hline 
      Sorting algorithms-Gnome sort      & 9        & 2 \\
        \hline 
      Forward difference      & 65        & 2 \\
        \hline 
      Palindrome detection      & 3        & 2 \\
        \hline 
      Horner's rule for polynomial evaluation      & 5        & 2 \\
        \hline 
      Continued fraction      & 257        & 2 \\
        \hline 
      Look-and-say sequence      & 17        & 2 \\
        \hline 
      Sparkline in unicode      & 513        & 2 \\
        \hline 
      Image noise      & 6        & 2 \\
        \hline 
      Nth root      & 136        & 2 \\
        \hline 
      Price fraction      & 17        & 2 \\
        \hline 
      Flatten a list      & 8193        & 2 \\
        \hline 
      Cycle detection      & 3        & 2 \\
        \hline 
      Sorting algorithms-Merge sort      & 16385        & 2 \\
        \hline 
      Feigenbaum constant calculation      & 3        & 2 \\
        \hline 
      Deconvolution-1D      & 3        & 2 \\
        \hline 
      Execute HQ9+      & 9        & 2 \\
        \hline 
      Catalan numbers      & 3        & 2 \\
        \hline 
      
  \end{tabular}
}
\end{table}
